Exploring Latent Semantic Factors to Find Useful Product Reviews

Online reviews provided by consumers are a valuable asset for e-Commerce platforms, influencing potential consumers in making purchasing decisions. However, these reviews are of varying quality, with the useful ones buried deep within a heap of non-informative reviews. In this work, we attempt to automatically identify review quality in terms of its helpfulness to the end consumers. In contrast to previous works in this domain exploiting a variety of syntactic and community-level features, we delve deep into the semantics of reviews as to what makes them useful, providing interpretable explanation for the same. We identify a set of consistency and semantic factors, all from the text, ratings, and timestamps of user-generated reviews, making our approach generalizable across all communities and domains. We explore review semantics in terms of several latent factors like the expertise of its author, his judgment about the fine-grained facets of the underlying product, and his writing style. These are cast into a Hidden Markov Model -- Latent Dirichlet Allocation (HMM-LDA) based model to jointly infer: (i) reviewer expertise, (ii) item facets, and (iii) review helpfulness. Large-scale experiments on five real-world datasets from Amazon show significant improvement over state-of-the-art baselines in predicting and ranking useful reviews.

==> compmodel.tex <==

\section{Overview}
\label{sec:overview}

\subsection{Model Dimensions}

Our approach is based on the intuition that there is a strong coupling between the \emph{facet preferences} of a user, her \emph{experience}, \emph{writing style} in reviews, and \emph{rating behavior}.
All of these factors jointly evolve with \emph{time} for a given user.
%For example, the preference of a user may change to the ``sci-fi'' genre with time, from the ``drama'' genre. Even within the same genre, the user may start appreciating intellectual movies like ``Gattaca'' and ``Inception'' more with time.

We model the user experience progression through discrete stages, so a state-transition model is natural. Once this decision is made, a Markovian model is the simplest, and thus natural choice. This is because the experience level of a user at the current instant $t$ depends on her experience level at the previous instant $t$-$1$. As experience levels are latent (not directly observable), a Hidden Markov Model is appropriate. Experience progression of a user depends on the following factors:

%In order to capture the \emph{experience progression} of a user with time, we consider a \emph{Hidden Markov Model} (HMM) where the experience level of the user is a \emph{latent} variable. The transition to an experience level at time $t$ depends on the experience level of the user at time $t$-$1$ and the following factors:

\squishlisttwo
\item \emph{Maturing rate} of the user which is modeled by her \emph{activity} in the community. The more engaged a user is in the community, 
the higher are the chances that she gains experience and advances in writing sophisticated reviews,
and develops taste to appreciate specific facets.
\item \emph{Facet preferences} of the user in terms of focusing on particular
facets of an item (e.g., narrative structure rather than special effects).
With increasing maturity, the taste for particular facets becomes more refined.
\item \emph{Writing style} of the user,  as expressed by the language model at her current level of experience. More sophisticated vocabulary and writing style indicates higher probability of progressing to a more mature level.
\item \emph{Time difference} between writing successive reviews. 
It is unlikely for the user's experience level to change from that of her last review in a short time span (within a few hours or days).
\item \emph{Experience level difference}: Since it is unlikely for a user to directly progress to say level $3$  from level $1$ without passing through level $2$, the model at each instant decides whether the user should stay at current level $l$, or progress to $l$+$1$.
%
%GW: I would drop the rest, as it is vague and not an explicit part of the our model anyway
\begin{comment}
The time required to say reach level $4$  from level $3$ is much less than that to reach level $2$ from level $1$, although few users would end up at level $4$ (on a scale of $1-5$ in the experience rating scale). This is implicitly captured in the model, and not encoded explicitly. A user spends the maximum time of his life cycle in the first two levels.
\end{comment}
\squishend

In order to learn the \emph{facet preferences} and \emph{language model} of a user at different levels of experience, we use \emph{Latent Dirichlet Allocation} (LDA). In this work, we assume each review to
refer to exactly one item. Therefore, the facet distribution of items is 
expressed in the facet distribution of the review documents.

We make the following assumptions for the generative process of writing a review by a user at time $t$ at  experience level $e_t$:

\squishlisttwo
\item A user has a distribution over \emph{facets},
where the facet preferences of the user depend on her experience level $e_t$.
\item A facet has a distribution over \emph{words} where the words used to describe a facet depend on the user's vocabulary at experience level $e_t$.
%(cf.  Table~\ref{tab:beerTopics}). 
%Table~\ref{tab:beerTopics} in Section~\ref{sec:experiments} shows the words 
%chosen by users at different levels of experience 
%to describe the facet ``taste'' in a beer community. 
Table \ref{tab:amazonTopics} shows salient words for two facets of
Amazon movie reviews at different levels of user experience, automatically extracted by our latent model.
The facets are latent, but we can interpret them as {\em plot/script} and
{\em narrative style}, respectively.
\squishend
%{\tt GW: todo: shrink Table , leave out some of the words !!!!! also need to 
%decide if table is better placed or in experiments section !!!!!}

\begin{table}
\small
\begin{tabular}{p{8.7cm}}
\toprule
\textbf{Level 1:} stupid people supposed wouldnt pass bizarre totally cant\\
\textbf{Level 2:}storyline acting time problems evil great times didnt money ended simply falls pretty\\
\textbf{Level 3:} movie plot good young epic rock tale believable acting\\
\textbf{Level 4:} script direction years amount fast primary attractive sense talent multiple demonstrates establish\\
\textbf{Level 5:} realism moments filmmaker visual perfect memorable recommended genius finish details defined talented visceral nostalgia\\
\midrule
\textbf{Level 1:} film will happy people back supposed good wouldnt cant\\
\textbf{Level 2:} storyline believable acting time stay laugh entire start funny\\
\textbf{Level 3 \& 4:} narrative cinema resemblance masterpiece crude undeniable admirable renowned seventies unpleasant myth nostalgic\\
\textbf{Level 5:} incisive delirious personages erudite affective dramatis nucleus cinematographic transcendence unerring peerless fevered\\
\bottomrule
\end{tabular}
\caption{Salient words for two facets at
five experience levels in movie reviews.}
\label{tab:amazonTopics}
         \vspace{-1.5em}
\end{table}

\noindent As a sanity check for our assumption of the coupling between user {\em experience}, {\em rating behavior}, {\em language} and {\em facet preferences}, we perform experimental studies reported next.

%GW: moved this to the begin of the section on the joint model
\begin{comment}
\subsection{Approach}

We start with an \emph{Author-Topic Model} (ATM)~\cite{rosenzviUAI2004} based on \emph{Latent Dirichlet Allocation} (LDA), where \emph{users} have a distribution over \emph{facets}, and facets have a distribution over \emph{words}. This is to find out the facets of interest to a user. These learnt facet preferences can be interpreted as latent item factors in the traditional \emph{Latent Factor Model} (LFM)~\cite{korenKDD2008}. However, the LFM is supervised as opposed to ATM. Incorporating supervision into the ATM to predict ratings is a non-trivial task. The user assigned ratings to items are continuous, and cannot be directly incorporated into a Multinomial distribution based ATM. This problem has been dealt with using Variational Inference in case of Supervised Topic Models~\cite{bleiNIPS2007}, where the flexibility comes at the cost of increasingly intractable inference. In our setting, we propose an \emph{Expectation-Maximization} framework (EM) to incorporate supervision, where the
latent facets are estimated in an \emph{E-Step} using \emph{Gibbs sampling} based inference; and \emph{Support Vector Regression} (SVR)~\cite{drucker97} is used in the \emph{M-Step} to learn the feature weights and predict ratings. Thereafter, we incorporate a layer for \emph{experience} in the ATM-LFM model, where the experience levels are drawn from a \emph{Hidden Markov Model} (HMM) in the \emph{E-Step}. The experience level transition depends on the evolution of the user \emph{learning rate}, \emph{facet preferences}, and \emph{writing style} over \emph{time}. The entire process is a supervised generative process of generating a review based on the experience level of a user hinged on HMM-LDA.
\end{comment}


==> relatedmodels.tex <==

%\section{Related Work}
%%%GW: we need a real related work section at the end of the paper - perhaps brief, but explicit 

%\section{Basic Models}
\section{Building Blocks of our Model}
%{\tt GW: or should we call these "Building Blocks of our Model" ?????}

Our model, presented in the next section, builds on and compares itself
against various baseline models as follows.

\subsection{Latent-Factor Recommendation}

According to the standard latent factor model (LFM)~\cite{korenKDD2008}, the rating assigned by a user $u$ to an item $i$ is given by:
\begin{equation}
\label{eq.1}
 rec(u, i) = \beta_g + \beta_u + \beta_i + \langle \alpha_u, \phi_i \rangle
\end{equation}

%{\tt GW: does <...,...> denote a scalar product ????? we need to be explicit here !!!!}
where $\langle .,. \rangle$ denotes a scalar product. $\beta_g$ is the average rating of all items by all users. $\beta_u$ is the offset of the average rating given by user $u$  from the global rating.
Likewise $\beta_i$ is the rating bias for item $i$. 
$\alpha_u$ and $\phi_i$ are the latent factors associated with user $u$ and item $i$, respectively. These latent factors are learned using gradient descent by minimizing the mean squared error ($MSE$) between observed ratings $r(u,i)$ and predicted ratings $rec(u,i)$:
$MSE = \frac{1}{|U|} \sum_{u,i \in U} (r(u,i) - rec(u, i))^2$

\subsection{Experience-based Latent-Factor Recommendation}

The most relevant baseline for our work is the ``user at learned rate'' model of ~\cite{mcauleyWWW2013},
which exploits that users at the same experience level have similar rating behavior even if their ratings are temporarily far apart. 
Experience of each user $u$ for item $i$ is modeled as a latent variable $e_{u,i} \in \{1...E\}$.
Different recommenders are learned for different experience levels. Therefore Equation~\ref{eq.1} is parameterized as:
\begin{equation}
\label{eq.3}
 rec_{e_{u,i}}(u, i) = \beta_g(e_{u,i}) + \beta_u(e_{u,i}) + \beta_i(e_{u,i}) + \langle \alpha_u(e_{u,i}), \phi_i(e_{u,i}) \rangle
\end{equation}

The parameters are learned using Limited Memory BFGS
%, a quasi-Newton method for non-linear optimization of problems with many variables, 
with the additional constraint that experience levels should be non-decreasing over the reviews written by a user over time. 

However, this is significantly different from our approach. All of these models work on the basis of only user {\em rating behavior}, and ignore the review texts completely. Additionally, the {\em smoothness} in the evolution of parameters between experience levels is enforced via $L_2$ regularization, and does not model the {\em natural} user maturing rate (via HMM) as in our model. Also note that in the above parametrization, an experience level is estimated for each user-item pair. However, it is rare that a user reviews the same item multiple times. In our approach, we instead trace the evolution of users, and not user-item pairs. 

%Most importantly, these models do not use the text of reviews.

\subsection{User-Facet Model}

In order to find the facets of interest to a user, \cite{rosenzviUAI2004} extends Latent Dirichlet Allocation (LDA) to include authorship information. 
Each document $d$ is considered to have a distribution over authors. 
We consider the special case where each document has exactly one author
$u$ associated with a Multinomial distribution $\theta_u$ over facets $Z$ with a symmetric Dirichlet prior $\alpha$. The facets have a Multinomial distribution $\phi_z$ over words $W$ drawn from a vocabulary $V$ with a symmetric Dirichlet prior $\beta$. %The generative process for a user writing a review is given by Algorithm~\ref{algo.1}.
%{\tt GW: do we really need - and want to keep - the algorithm here ?????}
Exact inference is not possible due to the intractable coupling between $\Theta$ and $\Phi$. Two ways for approximate inference are 
MCMC techniques like Collapsed Gibbs Sampling and Variational Inference.
The latter is typically much more complex and computationally expensive.
In our work, we thus use sampling.

\begin{comment}
\begin{algorithm}
\label{algo.1}
\small
\SetAlgoLined
\DontPrintSemicolon
\For {each user $u = 1, ... U$} {choose $\theta_u \sim  Dirichlet(\alpha)$} \;
\For {each topic $z = 1, ... K$} {choose $\phi_z \sim Dirichlet(\beta)$} \;
\For {each review $d = 1, ... D$} {
  Given the user $u_d$ \;
  \For {each word $i = 1, ... N_d$} {
    Conditioned on $u_d$ choose a topic $z_{d_i} \sim Multinomial(\theta_{u_d})$ \;
    Conditioned on $z_{d_i}$ choose a word $w_{d_i} \sim Multinomial(\phi_{z_{d_i}})$ \;
  }
}
\caption{Generative Process for User-Facet Model}
\label{algo.1}
\end{algorithm}
\end{comment}


\subsection{Supervised User-Facet Model}

The generative process described above is unsupervised and does not take the ratings in reviews into account. Supervision is difficult to build into MCMC sampling where ratings are continuous values, as in communities like {\small\tt newstrust.net}.
%and cannot be modeled by a Multinomial distribution. 
For discrete ratings, a review-specific Multinomial rating distribution $\pi_{d,r}$ can be learned as in~\cite{linCIKM2009, ramageKDD2011}. 
Discretizing the continuous ratings into buckets bypasses the problem to some extent, but results in loss of information. Other approaches~\cite{lakkarajuSDM2011, mcauleyRecSys2013, mukherjeeSDM2014} overcome this problem by learning the feature weights separately from the user-facet model.

%GW: I dismissed variational inference above, so we can drop this
\begin{comment}
A supervised version of the topic model using variational inference is proposed in~\cite{bleiNIPS2007}. It tackles the problem of coupling by removing some of the interactions altogether that makes the problem intractable; and learns a set of variational parameters that minimizes the $KL$ divergence between the approximate distribution and the true joint. However, the flexibility comes at the cost of increasingly intractable inference.
\end{comment}

\begin{figure}
  \vspace{-0.5em}
\centering
 \includegraphics[scale=0.3]{figure/SATRM.pdf}
  \caption{\small Supervised model for user facets and ratings.}
  \label{fig:1}
  \vspace{-1em}
\end{figure}
 
An elegant approach using Multinomial-Dirichlet Regression is proposed in~\cite{mimnoUAI2008} to incorporate arbitrary types of observed continuous or categorical features. Each facet $z$ is associated with a vector $\lambda_z$ whose dimension equals the number of features. Assuming $x_d$ is the feature vector for document $d$, the Dirichlet hyper-parameter $\alpha$ for the document-facet Multinomial distribution $\Theta$ is parametrized as $\alpha_{d,z}=exp(x_d^T\lambda_z)$. The model is trained using stochastic \emph{EM} which alternates between 1) sampling facet assignments from the posterior distribution conditioned on words and features, and 2) optimizing $\lambda$ given the facet assignments using L-BFGS.
Our approach, explained in the next section, follows a similar approach to couple 
the User-Facet Model and the Latent-Factor Recommendation Model (depicted in Figure~\ref{fig:1}).
%depicted in Figure~\ref{fig:1}.
%GW: no point in making this forward reference here

%{\tt GW: we sometimes talk about user-facet models (formerly author-topic 
%models) and sometimes about document-facet models - these are the same, but
%a reader may get confused !!!???}

==> relatedwork.tex <==
\section{Related Work}\label{sec:relWork}

Prior works on predicting review helpfulness~\cite{Kim:2006:AAR:1610075.1610135,Lu:2010:ESC:1772690.1772761} exploit shallow syntactic features to classify extremely opinionated reviews as not helpful. Similar features are also used in finding review spams~\cite{Liu2008, Liu2013}. Similarly, few other approaches utilize features like frequency of user posts, average ratings of users and items to distinguish between helpful and unhelpful reviews. Community-specific features with explicit user network are used in~\cite{Tang:2013:CRH:2507157.2507183,Lu:2010:ESC:1772690.1772761}. However, these shallow features do not analyze what the review is {\em about}, and, therefore, cannot {\em explain} why it should be helpful for a given product. 

Approaches proposed in~\cite{icdm2008,Kim:2006:AAR:1610075.1610135} also utilize item-specific meta-data like {\em explicit} item facets and product brands to decide the helpfulness of a review. However, these approaches heavily rely on a large number of meta-features which makes them less generalizable. Some of the related approaches~\cite{O'Mahony:2009:LRH:1639714.1639774,icdm2008} also identify {\em expertise} of a review's author as an important feature. However, they do not explicitly model the user expertise. 

Recent work in \cite{mcauleyWWW2013} studies the influence of rating behavior on evolving user experience. However, it does not consider the vocabulary and writing style of users in reviews, and their temporal progression. 
%In contrast, our work gains additional insights by considering the review texts to capture the facet preferences and experience progression. 
Our model for capturing user expertise draws motivation from~\cite{mukherjee2015jertm},\cite{mukherjee2016KDD},\cite{mcauleyWWW2013} with significant differences. Unlike prior works, the facet preferences in our model is conditioned only on the user expertise and not the user. This significantly reduces the dimensionality of the model making it more efficient; as well as the distributions are learned directly from minimizing the mean squared error for predictions, allowing all parameters to be coupled tightly, unlike in~\cite{mukherjee2015jertm}. 

User review text is also considered in Sentiment Analysis. These approaches aim to learns latent topics~\cite{linCIKM2009}, latent aspects and their ratings~\cite{lakkarajuSDM2011,wang2011,mcauleyrecsys2013}, and user-user interactions~\cite{West-etal:2014}. The author writing style is also used in \cite{mukherjeeSDM2014}. However, all of these prior approaches do not consider time or user expertise to capture the evolving writing style.

==> usecases.tex <==

\section{Use-Case Study}
\label{sec:usecases}

So far we have focused on traditional item recommendation for items like beers or movies. Now we switch to a different kind of items - newspapers and news articles - tapping into the NewsTrust online community ({\tt \small newstrust.net}). NewsTrust features news stories posted and reviewed by members, 
many of whom are professional journalists and content experts. Stories are reviewed based on their objectivity, rationality, and general quality of language to present an unbiased and balanced narrative of an event. The focus is on \emph{quality journalism}.

In our framework, each story is an item, which is rated and reviewed by a user. The facets are the underlying topic distribution of reviews, with topics being {\em Healthcare, Obama Administration, NSA}, etc. The facet preferences can be mapped to the (political) polarity of users in the news community. 

\noindent {\bf Recommending News Articles:}
Our first objective is to recommend news to readers catering to their facet preferences, viewpoints, and experience. We apply our joint model to this task, and compare the predicted ratings with the ones observed for withheld reviews in the NewsTrust community. The mean squared error (MSE) results are reported in Table~\ref{fig:MSE} in Section~\ref{sec:experiments}. Table~\ref{tab:newstrustTopics} shows salient examples of the vocabulary by users at different experience levels on the topic {\em US Election}.

\begin{table}
\small
\begin{tabular}{p{8cm}}
\toprule
\textbf{Level 1:} bad god religion iraq responsibility\\
\textbf{Level 2:} national reform live krugman questions clear jon led meaningful lives california powerful safety impacts\\
\textbf{Level 3:} health actions cuts medicare nov news points oil climate major jobs house high vote congressional spending unemployment strong taxes citizens events failure\\
\bottomrule
\end{tabular}
\caption{Salient words for the {\em illustrative} NewsTrust topic {\em US Election} at different experience levels.}
\label{tab:newstrustTopics}
\vspace{-1em}
\end{table}

%\paragraph{Identifying Experienced Users}

\begin{table}[t]
\begin{center}
 \begin{tabular}{lcc}
 \toprule
\bf{Models} & \bf{$F_1$} & \bf{$NDCG$}\\
\midrule
User at learned rate~\cite{mcauleyWWW2013} & 0.68 & 0.90 \\
Our model & 0.75 & 0.97 \\
\bottomrule
 \end{tabular}
\caption{Performance on identifying experienced users.}
\label{tab:ndcgUsers}
\end{center}
\vspace{-3em}
\end{table}

\noindent {\bf Identifying Experienced Users:}
Our second task is to find experienced members of this community, who have potential for being \emph{citizen journalists}. In order to find how good our model predicts the experience level of users, we consider the following as ground-truth for user experience. In NewsTrust, users have {\em Member Levels} calculated by the NewsTrust staff based on  community engagement, time in the community, other users' feedback on reviews, profile transparency, and manual validation.
We use these member levels to categorize users as {\em experienced} or {\em inexperienced}. This is treated as the ground truth for assessing the prediction and ranking quality of our model and the baseline ``user at learned rate'' model~\cite{mcauleyWWW2013}.
Table~\ref{tab:ndcgUsers} shows the $F_1$ scores of these two competitors.
We also computed the \emph{Normalized Discounted Cumulative Gain (NDCG)} \cite{Jarvelin:TOIS2002} 
%Kalervo Jarvelin, Jaana Kekalainen: Cumulated gain-based evaluation of IR 
%techniques. ACM Transactions on Information Systems 20(4), 422–446 (2002)
for the ranked lists of users generated by the two models. NDCG gives geometrically decreasing weights to predictions at various positions of ranked list:
{\small
$NDCG_p = \frac{DCG_p}{IDCG_p}$ where
$DCG_p = rel_1 + \sum_{i=2}^p \frac{rel_i}{\log_2 i}$
}

Here, $rel_i$ is the relevance ($0$ or $1$) of a result at position $i$. 
%DCG penalizes relevant items (\emph{experienced users}) appearing lower in 
%the rank list, where the graded relevance score is reduced logarithmically 
%proportional to the position of the result. 
%As the length of lists may vary for different queries, DCG scores are 
%normalized using the ideal score, IDCG where the results of a rank list are 
%sorted by relevance giving the maximum possible DCG score.

As Table~\ref{tab:ndcgUsers} shows, our model clearly outperforms the baseline model on both $F_1$ and $NDCG$.
